FoMoE: Breaking the Full-Replica Barrier with a Federation of MoEs

Pre-training Large Language Models (LLMs) typically demands large-scale infrastructure with tightly coupled hardware accelerators. Mixture-of-Experts (MoEs) architectures partially decouple model capacity from per-token compute. This efficiency alone does not make MoE training feasible over ordinary Internet links or loosely connected commodity hardware since active expert routing still assumes high-speed datacenter fabrics. Low-communication methods such as DiLoCo and Photon reduce synchronization frequency across distributed sites, mitigating bandwidth constraints, yet still require full model replicas at every site. This creates a mismatch: modern MoEs have sparse data paths, but their distributed training infrastructure remains communication-dense and memory-inefficient, limiting attempts to pool geographically distributed compute. In this work, we introduce FoMoE, a system that breaks the full-replica paradigm by partitioning expert layers across workers and skipping non-resident experts during local training. We demonstrate that FoMoE: (I) reduces communication costs by up to 1.42x over efficient baselines and 45.44x over Distributed Data Parallelism (DDP) via partial expert replication in controlled regimes; (II) achieves empirical throughput speedups of up to 1.4x through the skip-token mechanism; and (III) shows stable routing in the trained regimes and projects the communication/memory benefits to 100B-scale configurations through system modeling.

==> preamble/adapter.tex <==
\makeatletter

\def\@paper@title{Untitled}
\let\@paper@titlerunning\@empty
\let\@paper@keywords\@empty
\let\@paper@code\@empty
\let\@paper@plainauthors\@empty
\let\@paper@displayauthors\@empty
\let\@paper@displayaffils\@empty
\let\@paper@corrdisplay\@empty
\let\@paper@titlelogo\@empty
\def\paper@titlelogoheight{3.0em}
\def\paper@abstractfile{sections/abstract}
\newcounter{paper@affil}
\let\@neurips@authors\@empty
\let\@neurips@affils\@empty
\let\@neurips@corr\@empty
\let\@mlsys@authors\@empty
\let\@mlsys@affils\@empty
\let\@mlsys@corr\@empty
\newif\if@paper@firstauthor \@paper@firstauthortrue
\newif\if@paper@firstdisplayauthor \@paper@firstdisplayauthortrue
\newif\if@paper@hasequal \@paper@hasequalfalse
\newlength{\paper@titlecardinnerwidth}

\def\paper@titlecardpadding{0.45cm}
\def\paper@titlecardradius{10pt}

\definecolor{paperBrandCamlsysBlue}{HTML}{102344}
\definecolor{paperBrandCambridgeRed}{HTML}{EF2E31}
\definecolor{paperBrandCambridgeGold}{HTML}{FDDD04}
\colorlet{paperTitleBgCamlsys}{paperBrandCamlsysBlue!8!white}
\colorlet{paperTitleBgCambridgeGold}{paperBrandCambridgeGold!8!white}
\colorlet{paperTitleBgCambridge}{paperBrandCambridgeRed!3!paperTitleBgCambridgeGold}
\colorlet{paperTitleBgNeutral}{black!2!white}
\colorlet{paperTitleBg}{paperTitleBgCamlsys}
\definecolor{paperTitleFg}{HTML}{1F2328}
\definecolor{paperTitleMuted}{HTML}{4D5560}
\def\paper@titlebg@camlsys{camlsys}
\def\paper@titlebg@cambridge{cambridge}
\def\paper@titlebg@neutral{neutral}

\csdef{paper@sym@equal}{*}

\newcommand{\paperTitle}[1]{\def\@paper@title{#1}}
\newcommand{\paperKeywords}[1]{\def\@paper@keywords{#1}}
\newcommand{\paperCode}[1]{\def\@paper@code{#1}}
\newcommand{\paperAbstractFile}[1]{\def\paper@abstractfile{#1}}
\newcommand{\paperTitleLogo}[1]{\def\@paper@titlelogo{#1}}
\newcommand{\paperTitleLogoHeight}[1]{\def\paper@titlelogoheight{#1}}
\newcommand{\paperTitleBackground}[1]{  \edef\paper@titlebg@choice{#1}  \ifx\paper@titlebg@choice\paper@titlebg@camlsys
    \colorlet{paperTitleBg}{paperTitleBgCamlsys}  \else
    \ifx\paper@titlebg@choice\paper@titlebg@cambridge
      \colorlet{paperTitleBg}{paperTitleBgCambridge}    \else
      \ifx\paper@titlebg@choice\paper@titlebg@neutral
        \colorlet{paperTitleBg}{paperTitleBgNeutral}      \else
        \ClassWarning{paper}{Unknown title-card background theme `\paper@titlebg@choice'; keeping current theme}      \fi
    \fi
  \fi
}
\paperTitleBackground{\paper@titlebg}
\newcommand{\paperTitleRunning}[1]{  \def\@paper@titlerunning{#1}  \ifpaper@mlsys \mlsystitlerunning{#1}\fi  }

\newcommand{\addAffiliation}[2]{  \stepcounter{paper@affil}  \csedef{paper@affil@#1}{\thepaper@affil}  \ifnum\value{paper@affil}>\@ne \appto\@paper@displayaffils{\quad}\fi
  \protected@eappto\@paper@displayaffils{\noexpand\textsuperscript{\arabic{paper@affil}}}  \appto\@paper@displayaffils{#2}  \ifpaper@neurips
    \ifnum\value{paper@affil}>\@ne \appto\@neurips@affils{\quad}\fi
    \protected@eappto\@neurips@affils{\noexpand\textsuperscript{\arabic{paper@affil}}}    \appto\@neurips@affils{#2}  \fi
  \ifpaper@mlsys
    \appto\@mlsys@affils{\mlsysaffiliation{#1}{#2}}  \fi
}

\newcommand{\paper@resolvekey}[1]{  \ifcsdef{paper@sym@#1}{    \ifstrequal{#1}{equal}{\@paper@hasequaltrue}{}    \protected@eappto\@paper@syms{\csuse{paper@sym@#1}}  }{    \ifcsdef{paper@affil@#1}{      \ifx\@paper@nums\@empty\else\appto\@paper@nums{,}\fi
      \protected@eappto\@paper@nums{\csuse{paper@affil@#1}}    }{\ClassWarning{paper}{\noexpand\addAuthor: unknown key `#1'}}  }}
\newcommand{\addAuthor}[2]{  \ifx\@paper@plainauthors\@empty
    \appto\@paper@plainauthors{#1}  \else
    \appto\@paper@plainauthors{, #1}  \fi
  \let\@paper@nums\@empty \let\@paper@syms\@empty
  \forcsvlist{\paper@resolvekey}{#2}  \if@paper@firstdisplayauthor\else\appto\@paper@displayauthors{,\space}\fi
  \appto\@paper@displayauthors{#1}  \protected@eappto\@paper@displayauthors{\noexpand\textsuperscript{\@paper@nums\@paper@syms}}  \@paper@firstdisplayauthorfalse
  \ifpaper@neurips
    \if@paper@firstauthor\else\appto\@neurips@authors{,\space}\fi
    \appto\@neurips@authors{#1}    \protected@eappto\@neurips@authors{\noexpand\textsuperscript{\@paper@nums\@paper@syms}}    \@paper@firstauthorfalse
  \fi
  \ifpaper@mlsys
    \appto\@mlsys@authors{\mlsysauthor{#1}{#2}}  \fi
}

\newcommand{\correspondingAuthor}[2]{  \appto\@paper@corrdisplay{#1 \texttt{<#2>}}  \ifpaper@neurips \appto\@neurips@corr{\thanks{Correspondence to: #1 \texttt{<#2>}}}\fi
  \ifpaper@mlsys   \appto\@mlsys@corr{\mlsyscorrespondingauthor{#1}{#2}}\fi
}

\newcommand{\paper@setneuripspdfauthor}{  \hypersetup{pdfauthor={\@paper@plainauthors}}}
\newcommand{\paper@setmlsyspdfauthor}{  \hypersetup{pdfauthor={\@paper@plainauthors}}}
\newcommand{\paper@setpdfmetadata}{  \@ifpackageloaded{hyperref}{    \hypersetup{pdftitle={\@paper@title}}    \ifx\@paper@keywords\@empty\else
      \hypersetup{pdfkeywords={\@paper@keywords}}    \fi
    \ifpaper@neurips
      \paper@setneuripspdfauthor
    \fi
    \ifpaper@mlsys
      \paper@setmlsyspdfauthor
    \fi
  }{}}

\newcommand{\paper@titleLogoGraphic}{  \IfFileExists{\@paper@titlelogo}{    \includegraphics[height=\paper@titlelogoheight,width=\linewidth,keepaspectratio]{\@paper@titlelogo}  }{    \ClassWarning{paper}{Title logo `\@paper@titlelogo' not found}    \fbox{\rule{0pt}{\paper@titlelogoheight}\textsf{\small logo}}  }}

\newcommand{\paper@titleLine}{  \ifx\@paper@titlelogo\@empty
    {\raggedright\sffamily\bfseries\huge\color{paperTitleFg}\@paper@title\par}  \else
    \noindent
    \begin{minipage}[c]{0.14\linewidth}
      \centering\paper@titleLogoGraphic
    \end{minipage}\hspace{0.03\linewidth}    \begin{minipage}[c]{0.81\linewidth}
      {\raggedright\sffamily\bfseries\huge\color{paperTitleFg}\@paper@title\par}    \end{minipage}\par
  \fi
}

\newcommand{\paper@identityBlock}{  \ifx\@paper@displayauthors\@empty\else
    {\sffamily\bfseries\large\color{paperTitleFg}\@paper@displayauthors\par}  \fi
  \ifx\@paper@displayaffils\@empty\else
    \vspace{0.10cm}    {\small\color{paperTitleMuted}\@paper@displayaffils\par}  \fi
}

\newcommand{\paper@metadataText}{  \if@paper@hasequal
    \textsuperscript{*}Equal contribution.\par
  \fi
  \ifx\@paper@corrdisplay\@empty\else
    {\sffamily\bfseries Correspondence:} \@paper@corrdisplay\par
  \fi
  \ifx\@paper@keywords\@empty\else
    {\sffamily\bfseries Keywords:} \@paper@keywords\par
  \fi
  \ifx\@paper@code\@empty\else
    {\sffamily\bfseries Code:} \@paper@code\par
  \fi
}

\newcommand{\paper@metadataRow}{  \noindent
  \begin{minipage}[t]{0.7\linewidth}
    {\small\color{paperTitleMuted}\paper@metadataText}  \end{minipage}\par
}

\newcommand{\paper@titlecardLogoOverlay}{  \ifx\paper@logos\paper@logos@none\else
    \node[
      anchor=south east,
      inner sep=0pt,
      outer sep=0pt,
      xshift=-\paper@titlecardpadding,
      yshift=\paper@titlecardpadding
    ] at (paperTitleCardNode.south east) {\paperLogoStrip};  \fi
}

\newcommand{\paper@titlecard}{  \begingroup
    \setlength{\paper@titlecardinnerwidth}{\dimexpr\linewidth-\paper@titlecardpadding-\paper@titlecardpadding\relax}    \noindent
    \begin{tikzpicture}
      \node[
        fill=paperTitleBg,
        rounded corners=\paper@titlecardradius,
        inner sep=\paper@titlecardpadding,
        outer sep=0pt,
        text width=\paper@titlecardinnerwidth,
        align=left
      ] (paperTitleCardNode) {        \begin{minipage}{\paper@titlecardinnerwidth}
          \setlength{\parindent}{0pt}          \setlength{\parskip}{0pt}          \raggedright
          \paper@titleLine
          \vspace{0.30cm}          \paper@identityBlock
          \vspace{0.38cm}          {\small\color{paperTitleFg}{\sffamily\bfseries Abstract.}\space\input{\paper@abstractfile}\par}          \vspace{0.42cm}          \paper@metadataRow
        \end{minipage}      };      \paper@titlecardLogoOverlay
    \end{tikzpicture}    \par\vspace{0.35cm}  \endgroup
}

\newcommand{\paper@setmlsysrunninghead}{  \ifx\@paper@titlerunning\@empty
    \gdef\@mlsystitlerunning{\@paper@title}  \else
    \gdef\@mlsystitlerunning{\@paper@titlerunning}  \fi
  \chead{\small\bf\@mlsystitlerunning}  \thispagestyle{empty}}

\newcommand{\paper@mlsysNotice}{  {\let\thefootnote\relax\footnotetext{\hspace*{-\footnotesep}\Notice@String}}}

\newcommand{\makepapertitle}{  \paper@setpdfmetadata
  \ifpaper@neurips
    \par
    \begingroup
      \thispagestyle{empty}      \paper@titlecard
      \@notice
    \endgroup
  \fi
  \ifpaper@mlsys
    \paper@setmlsysrunninghead
    \twocolumn[      \paper@titlecard
      \vskip 0.18in
    ]    \paper@mlsysNotice
  \fi
}

\makeatother


==> preamble/format.tex <==
\makeatletter

\newif\ifpaper@neurips
\newif\ifpaper@mlsys
\newif\ifpaper@twocolumn

\def\paper@@neurips{neurips}
\def\paper@@mlsys{mlsys}
\ifx\paper@format\paper@@mlsys
  \paper@mlsystrue
\else
  \ifx\paper@format\paper@@neurips
    \paper@neuripstrue
  \else
    \ClassError{paper}{Unknown format `\paper@format'; use format=neurips or format=mlsys}{}  \fi
\fi

\ifpaper@neurips
  \paper@twocolumnfalse
  \RequirePackage[preprint]{neurips_2026}        \def\paperbibstyle{plainnat}\fi

\ifpaper@mlsys
  \paper@twocolumntrue
    \providecommand{\theHalgorithm}{\arabic{algorithm}}  \RequirePackage[accepted]{mlsys2026}  \def\paperbibstyle{mlsys2026}\fi

\makeatother


==> preamble/logos.tex <==
\makeatletter

\newcommand{\paper@logoheight}{13mm}

\newcommand{\paper@logo}[2]{  \raisebox{-0.5\height}{    \IfFileExists{branding/#1.pdf}{\includegraphics[height=\paper@logoheight]{branding/#1.pdf}}{    \IfFileExists{branding/#1.png}{\includegraphics[height=\paper@logoheight]{branding/#1.png}}{    \IfFileExists{branding/#1.jpg}{\includegraphics[height=\paper@logoheight]{branding/#1.jpg}}{    \fbox{\rule[-2.5mm]{0pt}{\paper@logoheight}\textsf{\small\,#2\,}}}}}  }}

\newcommand{\paper@logoOr}[3]{  \IfFileExists{branding/#1.pdf}{\paper@logo{#1}{#3}}{  \IfFileExists{branding/#1.png}{\paper@logo{#1}{#3}}{  \IfFileExists{branding/#1.jpg}{\paper@logo{#1}{#3}}{  \paper@logo{#2}{#3}}}}}

\def\paper@logos@none{none}
\def\paper@logos@cc{camlsys-cambridge}
\def\paper@logos@ccf{camlsys-cambridge-flower}

\newcommand{\paperLogoStrip}{  \ifx\paper@logos\paper@logos@none\else
    \begingroup
      \renewcommand{\paper@logoheight}{13mm}      \ifx\paper@logos\paper@logos@ccf
        \paper@logoOr{camlsys}{big_camlsys_logo}{CaMLSys}\hspace{0.55em}        \paper@logo{cambridge}{University of Cambridge}\hspace{0.55em}        \paper@logo{flower}{Flower Labs}      \else
        \paper@logoOr{camlsys}{big_camlsys_logo}{CaMLSys}\hspace{0.55em}        \paper@logo{cambridge}{University of Cambridge}      \fi
    \endgroup
  \fi
}

\newcommand{\logoHeader}{  \ifx\paper@logos\paper@logos@none\else
    \begin{center}      \noindent\begin{minipage}{\textwidth}\centering
        \ifx\paper@logos\paper@logos@ccf
          \paper@logoOr{camlsys}{big_camlsys_logo}{CaMLSys}\hfill
          \paper@logo{cambridge}{University of Cambridge}\hfill
          \paper@logo{flower}{Flower Labs}        \else
          \paper@logoOr{camlsys}{big_camlsys_logo}{CaMLSys}\hfill
          \paper@logo{cambridge}{University of Cambridge}        \fi
      \end{minipage}    \end{center}    \vspace{0.5\baselineskip}  \fi
}

\makeatother


==> preamble/macros.tex <==
\makeatletter

\graphicspath{{figures/}{figures/plots/}{figures/diagrams/}{figures/tikz/}{branding/}}

\newenvironment{widefigure}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{figure*}[#1]\else \@nameuse{figure}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endfigure*}\else \@nameuse{endfigure}\fi}
\newenvironment{widetable}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{table*}[#1]\else \@nameuse{table}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endtable*}\else \@nameuse{endtable}\fi}

\newcommand{\PaperIfTwoColumn}[2]{\ifpaper@twocolumn #1\else #2\fi}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\etal}{et~al.\xspace}
\newcommand{\dashes}{---\xspace}

\newcommand{\method}{\texttt{FoMoE}\xspace}
\newcommand{\diloco}{\texttt{DiLoCo}\xspace}
\newcommand{\localsgd}{\texttt{LocalSGD}\xspace}
\newcommand{\localadamw}{\texttt{LocalAdamW}\xspace}
\newcommand{\localadam}{\texttt{LocalAdam}\xspace}
\newcommand{\desloc}{\texttt{DES-LOC}\xspace}
\newcommand{\photon}{\texttt{Photon}\xspace}
\newcommand{\llms}{\texttt{LLMs}\xspace}
\newcommand{\moes}{\texttt{MoEs}\xspace}
\newcommand{\moe}{\texttt{MoE}\xspace}
\newcommand{\flop}{\texttt{FLOP}\xspace}
\newcommand{\flops}{\texttt{FLOPs}\xspace}
\newcommand{\wan}{\texttt{WAN}\xspace}
\newcommand{\wans}{\texttt{WANs}\xspace}
\newcommand{\vms}{\texttt{VMs}\xspace}
\newcommand{\vm}{\texttt{VM}\xspace}
\newcommand{\dc}{\texttt{DC}\xspace}
\newcommand{\ffn}{\texttt{FFN}\xspace}
\newcommand{\ffns}{\texttt{FFNs}\xspace}
\newcommand{\silu}{\texttt{SiLU}\xspace}
\newcommand{\dept}{\texttt{DEPT}\xspace}
\newcommand{\adamw}{\texttt{AdamW}\xspace}
\newcommand{\fedopt}{\texttt{FedOPT}\xspace}
\newcommand{\completep}{\texttt{CompleteP}\xspace}
\newcommand{\mup}{$\mu$\texttt{P}\xspace}

\providecommand{\todo}[1]{{\normalfont\color{red}\,[TODO: #1]\,}}
\newcommand{\note}[2]{{\normalfont\color{blue}\,[#1: #2]\,}}
\newcommand{\ls}[1]{\todo{Lorenzo: #1}}
\newcommand{\aj}[1]{\todo{Andrej: #1}}
\newcommand{\jc}[1]{\todo{Jamie: #1}}
\newcommand{\wz}[1]{\textcolor{violet}{\textbf{Wanru:} #1}}

\makeatother


==> preamble/packages.tex <==
\makeatletter

\RequirePackage{etoolbox}   
\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[utf8]{inputenc}
  \RequirePackage[T1]{fontenc}
\fi

\RequirePackage{graphicx}
\RequirePackage{booktabs}        \RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsfonts}
\RequirePackage{mathtools}
\RequirePackage{microtype}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{nicefrac}
\RequirePackage{xspace}
\RequirePackage{siunitx}
\sisetup{round-mode=places, round-precision=2, per-mode=symbol, per-symbol=p}
\@ifundefined{bit}{\DeclareSIUnit\bit{b}}{}
\RequirePackage{csvsimple}       \RequirePackage{pgfplots}\pgfplotsset{compat=1.18}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,positioning,shapes,shapes.geometric,calc,fit,backgrounds,shadows}
\RequirePackage{standalone}      \RequirePackage{subcaption}      \RequirePackage{rotating}
\captionsetup{compatibility=false, labelfont=bf, font=small}
\RequirePackage{multirow}
\RequirePackage{multicol}
\RequirePackage{paralist}
\RequirePackage{setspace}
\RequirePackage{float}
\RequirePackage{placeins}
\RequirePackage{cuted}
\RequirePackage[toc, title]{appendix}
\RequirePackage{minitoc}

\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\providecommand{\theHalgorithm}{\arabic{algorithm}}
\providecommand{\Require}{\REQUIRE}
\providecommand{\Ensure}{\ENSURE}
\providecommand{\State}{\STATE}
\providecommand{\Statex}{\item[]}
\providecommand{\If}[1]{\IF{#1}}
\providecommand{\Else}{\ELSE}
\providecommand{\ElsIf}[1]{\ELSIF{#1}}
\providecommand{\EndIf}{\ENDIF}
\providecommand{\For}[1]{\FOR{#1}}
\providecommand{\ForAll}[1]{\FORALL{#1}}
\providecommand{\EndFor}{\ENDFOR}
\providecommand{\While}[1]{\WHILE{#1}}
\providecommand{\EndWhile}{\ENDWHILE}
\providecommand{\Loop}{\LOOP}
\providecommand{\EndLoop}{\ENDLOOP}
\providecommand{\Repeat}{\REPEAT}
\providecommand{\Until}[1]{\UNTIL{#1}}
\providecommand{\Function}[1]{\FUNCTION{#1}}
\providecommand{\EndFunction}{\ENDFUNCTION}

\RequirePackage{xurl}
\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\definecolor{paperlink}{rgb}{0.10,0.20,0.55}
\hypersetup{colorlinks=true, linkcolor=paperlink, citecolor=paperlink, urlcolor=paperlink, breaklinks=true}
\RequirePackage[capitalise, nameinlink]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Sec.}{Secs.}
\crefname{subsection}{Sec.}{Secs.}
\Crefname{subsection}{Sec.}{Secs.}
\crefname{subsubsection}{Sec.}{Secs.}
\Crefname{subsubsection}{Sec.}{Secs.}
\crefname{appendix}{App.}{Apps.}
\Crefname{appendix}{App.}{Apps.}
\crefname{subappendix}{App.}{Apps.}
\Crefname{subappendix}{App.}{Apps.}
\crefname{subsubappendix}{App.}{Apps.}
\Crefname{subsubappendix}{App.}{Apps.}
\crefname{subsubsubappendix}{App.}{Apps.}
\Crefname{subsubsubappendix}{App.}{Apps.}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{subfigure}{Fig.}{Figs.}
\Crefname{subfigure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Tab.}{Tabs.}
\crefname{subtable}{Tab.}{Tabs.}
\Crefname{subtable}{Tab.}{Tabs.}
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algorithm}{Alg.}{Algs.}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}

\makeatother


==> sections/abstract.tex <==
Pre-training Large Language Models (\llms) typically demands large-scale infrastructure with tightly coupled hardware accelerators. Mixture-of-Experts (\moes) architectures partially decouple model capacity from per-token compute. This efficiency alone does not make MoE training feasible over ordinary Internet links or loosely connected commodity hardware since active expert routing still assumes high-speed datacenter fabrics. Low-communication methods such as \diloco and \photon reduce synchronization frequency across distributed sites, mitigating bandwidth constraints, yet still require \emph{full model replicas} at every site. This creates a mismatch: modern \moes have sparse data paths, but their distributed training infrastructure remains communication-dense and memory-inefficient, limiting attempts to pool geographically distributed compute. In this work, we introduce \method, a system that breaks the full-replica paradigm by partitioning expert layers across workers and skipping non-resident experts during local training. We demonstrate that \method: (I) reduces communication costs by up to $1.42\times$ over efficient baselines and $45.44\times$ over Distributed Data Parallelism~(\texttt{DDP}) via partial expert replication in controlled regimes; (II) achieves empirical throughput speedups of up to $1.4\times$ through the ``skip-token'' mechanism; and (III) shows stable routing in the trained regimes and projects the communication/memory benefits to $100$B-scale configurations through system modeling.

